Cubic Halo Bias in Eulerian and Lagrangian Space

Predictions of the next-to-leading order, i.e. one-loop, halo power spectra depend on local and non-local bias parameters up to cubic order. The linear bias parameter can be estimated from the large scale limit of the halo-matter power spectrum, and the second order bias parameters from the large scale, tree-level, bispectrum. Cubic operators would naturally be quantified using the tree-level trispectrum. As the latter is computationally expensive, we extent the quadratic field method proposed in Schmittfull et al. 2014 to cubic fields in order to estimate cubic bias parameters. We cross-correlate a basis set of cubic bias operators with the halo field and express the result in terms of the cross-spectra of these operators in order to cancel cosmic variance. We obtain significant detections of local and non-local cubic bias parameters, which are partially in tension with predictions based on local Lagrangian bias schemes. We directly measure the Lagrangian bias parameters of the protohaloes associated with our halo sample and clearly detect a non-local quadratic term in Lagrangian space. We do not find a clear detection of non-local cubic Lagrangian terms for low mass bins, but there is some mild evidence for their presence for the highest mass bin. While the method presented here focuses on cubic bias parameters, the approach could also be applied to quantifications of cubic primordial non-Gaussianity.

==> bib.tex <==
%\cite{Schmittfull:2014tca}
\bibitem{Schmittfull:2014tca}
  M.~Schmittfull, T.~Baldauf and U.~Seljak,
  \emph{Near optimal bispectrum estimators for large-scale structure,}
  Phys.\ Rev.\ D {\bf 91} (2015) no.4,  043530
  doi:10.1103/PhysRevD.91.043530
  [arXiv:1411.6595 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.91.043530;%%



  
 %\cite{Carrasco:2012cv}
\bibitem{Carrasco:2012cv}
  J.~J.~M.~Carrasco, M.~P.~Hertzberg and L.~Senatore,
  \emph{The Effective Field Theory of Cosmological Large Scale Structures},
  JHEP {\bf 1209} (2012) 082
  doi:10.1007/JHEP09(2012)082
  [arXiv:1206.2926 [astro-ph.CO]].
  %%CITATION = doi:10.1007/JHEP09(2012)082;%%
  %174 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Baumann:2010tm}
\bibitem{Baumann:2010tm}
  D.~Baumann, A.~Nicolis, L.~Senatore and M.~Zaldarriaga,
  \emph{Cosmological Non-Linearities as an Effective Fluid},
  JCAP {\bf 1207} (2012) 051
  doi:10.1088/1475-7516/2012/07/051
  [arXiv:1004.2488 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2012/07/051;%%
  %206 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Porto:2013qua}
\bibitem{Porto:2013qua}
  R.~A.~Porto, L.~Senatore and M.~Zaldarriaga,
  \emph{The Lagrangian-space Effective Field Theory of Large Scale Structures},
  JCAP {\bf 1405} (2014) 022
  doi:10.1088/1475-7516/2014/05/022
  [arXiv:1311.2168 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2014/05/022;%%
  %86 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Senatore:2014via}
\bibitem{Senatore:2014via}
  L.~Senatore and M.~Zaldarriaga,
  \emph{The IR-resummed Effective Field Theory of Large Scale Structures},
  JCAP {\bf 1502} (2015) no.02,  013
  doi:10.1088/1475-7516/2015/02/013
  [arXiv:1404.5954 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2015/02/013;%%
  %69 citations counted in INSPIRE as of 20 Jan 2018
  
%\cite{Baldauf:2014qfa}
\bibitem{Baldauf:2014qfa}
  T.~Baldauf, L.~Mercolli, M.~Mirbabayi and E.~Pajer,
  \emph{The Bispectrum in the Effective Field Theory of Large Scale Structure},
  JCAP {\bf 1505} (2015) no.05,  007
  doi:10.1088/1475-7516/2015/05/007
  [arXiv:1406.4135 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2015/05/007;%%
  %55 citations counted in INSPIRE as of 20 Jan 2018


%\cite{Angulo:2014tfa}
\bibitem{Angulo:2014tfa}
  R.~E.~Angulo, S.~Foreman, M.~Schmittfull and L.~Senatore,
  \emph{The One-Loop Matter Bispectrum in the Effective Field Theory of Large Scale Structures},
  JCAP {\bf 1510} (2015) no.10,  039
  doi:10.1088/1475-7516/2015/10/039
  [arXiv:1406.4143 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2015/10/039;%%
  %44 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Baldauf:2015aha}
\bibitem{Baldauf:2015aha}
  T.~Baldauf, L.~Mercolli and M.~Zaldarriaga,
  \emph{Effective field theory of large scale structure at two loops: The apparent scale dependence of the speed of sound,}
  Phys.\ Rev.\ D {\bf 92} (2015) no.12,  123007
  doi:10.1103/PhysRevD.92.123007
  [arXiv:1507.02256 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.92.123007;%%
  %38 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Carrasco:2013sva}
\bibitem{Carrasco:2013sva}
  J.~J.~M.~Carrasco, S.~Foreman, D.~Green and L.~Senatore,
  \emph{The 2-loop matter power spectrum and the IR-safe integrand,}
  JCAP {\bf 1407} (2014) 056
  doi:10.1088/1475-7516/2014/07/056
  [arXiv:1304.4946 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2014/07/056;%%
  %59 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Bertolini:2016bmt}
\bibitem{Bertolini:2016bmt}
  D.~Bertolini, K.~Schutz, M.~P.~Solon and K.~M.~Zurek,
  \emph{The Trispectrum in the Effective Field Theory of Large Scale Structure,}
  JCAP {\bf 1606} (2016) no.06,  052
  doi:10.1088/1475-7516/2016/06/052
  [arXiv:1604.01770 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2016/06/052;%%
  %14 citations counted in INSPIRE as of 20 Jan 2018


%\cite{Lazeyras:2017hxw}
\bibitem{Lazeyras:2017hxw}
  T.~Lazeyras and F.~Schmidt,
  \emph{Beyond LIMD bias: a measurement of the complete set of third-order halo bias parameters,}
  arXiv:1712.07531 [astro-ph.CO].

%\cite{Ade:2015ava}
\bibitem{Ade:2015ava}
  P.~A.~R.~Ade {\it et al.} [Planck Collaboration],
  \emph{Planck 2015 results. XVII. Constraints on primordial non-Gaussianity,}
  Astron.\ Astrophys.\  {\bf 594} (2016) A17
  doi:10.1051/0004-6361/201525836
  [arXiv:1502.01592 [astro-ph.CO]].
  %%CITATION = doi:10.1051/0004-6361/201525836;%%


%\cite{Assassi:2014fva}
\bibitem{Assassi:2014fva}
  V.~Assassi, D.~Baumann, D.~Green and M.~Zaldarriaga,
  \emph{Renormalized Halo Bias,}
  JCAP {\bf 1408} (2014) 056
  doi:10.1088/1475-7516/2014/08/056
  [arXiv:1402.5916 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2014/08/056;%%


\bibitem{Schmidt2012Peak-BackgroundClustering}
    F.~Schmidt, D.~Jeong, V.~Desjacques
    \emph{Peak-Background Split, Renormalization, and Galaxy Clustering}
    {2012}
    doi: 10.1103/PhysRevD.88.023515
    [arXiv: 1212.0868]

%\cite{Modi:2016dah}
\bibitem{Modi:2016dah}
  C.~Modi, E.~Castorina and U.~Seljak,
  \emph{Halo bias in Lagrangian Space: Estimators and theoretical predictions},
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 472} (2017) no.4,  3959
  doi:10.1093/mnras/stx2148
  [arXiv:1612.01621 [astro-ph.CO]].
  %%CITATION = doi:10.1093/mnras/stx2148;%%
  %11 citations counted in INSPIRE as of 07 Feb 2018

%\cite{Baldauf:2010d}
%\bibitem{Baldauf:2010d}
%  T.~Baldauf, E.~Castorina and U.~Seljak,
%  \emph{Primordial non-Gaussianity in the Bispectrum of the Halo Density Field}
%  JCAP {\bf 04} (2011) 006
%  doi:10.1088/1475-7516/2011/04/006
%  [arXiv:1011.1513 [astro-ph.CO]].


%\cite{Sheth:1999mn}
\bibitem{Sheth:1999mn}
  R.~K.~Sheth and G.~Tormen,
  \emph{Large scale bias and the peak background split,}
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 308} (1999) 119
  doi:10.1046/j.1365-8711.1999.02692.x
  [astro-ph/9901122].
  %%CITATION = doi:10.1046/j.1365-8711.1999.02692.x;%%
  %1671 citations counted in INSPIRE as of 18 Jan 2018
% Also, please have only one work for each \bibitem.

%\cite{Chan:2012jj}
\bibitem{Chan:2012jj}
  K.~C.~Chan, R.~Scoccimarro and R.~K.~Sheth,
  \emph{Gravity and Large-Scale Non-local Bias,}
  Phys.\ Rev.\ D {\bf 85} (2012) 083509
  doi:10.1103/PhysRevD.85.083509
  [arXiv:1201.3614 [astro-ph.CO]].


%\cite{Vlah:2016bcl}
\bibitem{Vlah:2016bcl}
  Z.~Vlah, E.~Castorina and M.~White,
  \emph{The Gaussian streaming model and convolution Lagrangian effective field theory,}
  JCAP {\bf 1612} (2016) no.12,  007
  doi:10.1088/1475-7516/2016/12/007
  [arXiv:1609.02908 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2016/12/007;%%
  %11 citations counted in INSPIRE as of 20 Jan 2018
  
  
\bibitem{McDonald2009}}
P.~McDonald and A.~Roy,
\emph{Clustering of dark matter tracers: generalizing bias for the coming era of precision LSS}
 2009, Journal of Cosmology and Astroparticle
Physics, 2009, 020

%\cite{Senatore:2014eva}
\bibitem{Senatore:2014eva}
  L.~Senatore,
  \emph{Bias in the Effective Field Theory of Large Scale Structures,}
  JCAP {\bf 1511} (2015) no.11,  007
  doi:10.1088/1475-7516/2015/11/007
  [arXiv:1406.7843 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2015/11/007;%%
  %48 citations counted in INSPIRE as of 20 Jan 2018

%\cite{Fry:1992vr}
\bibitem{Fry:1992vr}
  J.~N.~Fry and E.~Gaztanaga,
  \emph{Biasing and hierarchical statistics in large scale structure,}
  Astrophys.\ J.\  {\bf 413} (1993) 447
  doi:10.1086/173015
  [astro-ph/9302009].
  %%CITATION = doi:10.1086/173015;%%
  %367 citations counted in INSPIRE as of 20 Jan 2018
  
 
\bibitem{Baldauf}	
T.~Baldauf, U.~Seljak; V.~Desjacques; P.~McDonald
\emph{ Evidence for quadratic tidal tensor bias from the halo bispectrum
Authors}

  
%\cite{Fujita:2016dne}
\bibitem{Fujita:2016dne}
  T.~Fujita, V.~Mauerhofer, L.~Senatore, Z.~Vlah and R.~Angulo,
  Very Massive Tracers and Higher Derivative Biases,''
  arXiv:1609.00717 [astro-ph.CO].
  %%CITATION = ARXIV:1609.00717;%%
  %10 citations counted in INSPIRE as of 11 Feb 2018
  
  %\cite{Angulo:2015eqa}
\bibitem{Angulo:2015eqa}
  R.~Angulo, M.~Fasiello, L.~Senatore and Z.~Vlah,
  %``On the Statistics of Biased Tracers in the Effective Field Theory of Large Scale Structures,''
  JCAP {\bf 1509} (2015) no.09,  029
  doi:10.1088/1475-7516/2015/09/029, 10.1088/1475-7516/2015/9/029
  [arXiv:1503.08826 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2015/09/029, 10.1088/1475-7516/2015/9/029;%%
  %36 citations counted in INSPIRE as of 13 Feb 2018

%\cite{Pajer:2013jj}
\bibitem{Pajer:2013jj}
  E.~Pajer and M.~Zaldarriaga,
  \emph{On the Renormalization of the Effective Field Theory of Large Scale Structures,}
  JCAP {\bf 1308} (2013) 037
  doi:10.1088/1475-7516/2013/08/037
  [arXiv:1301.7182 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2013/08/037;%%
  %76 citations counted in INSPIRE as of 21 Jan 2018

%\cite{Schmittfull:2014tca}
\bibitem{Schmittfull:2014tca}
  M.~Schmittfull, T.~Baldauf and U.~Seljak,
  \emph{Near optimal bispectrum estimators for large-scale structure,}
  Phys.\ Rev.\ D {\bf 91} (2015) no.4,  043530
  doi:10.1103/PhysRevD.91.043530
  [arXiv:1411.6595 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.91.043530;%%
  %16 citations counted in INSPIRE as of 20 Jan 2018
  
  
  %\cite{Saito:2014qha}
\bibitem{Saito:2014qha}
  S.~Saito, T.~Baldauf, Z.~Vlah, U.~Seljak, T.~Okumura and P.~McDonald,
  \emph{Understanding higher-order nonlocal halo bias at large scales by combining the power spectrum with the bispectrum,}
  Phys.\ Rev.\ D {\bf 90} (2014) no.12,  123522
  doi:10.1103/PhysRevD.90.123522
  [arXiv:1405.1447 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.90.123522;%%
  %58 citations counted in INSPIRE as of 21 Jan 2018
  
%\cite{Scoccimarro:2011pz}
\bibitem{Scoccimarro:2011pz}
  R.~Scoccimarro, L.~Hui, M.~Manera and K.~C.~Chan,
  %``Large-scale Bias and Efficient Generation of Initial Conditions for Non-Local Primordial Non-Gaussianity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 083002
  doi:10.1103/PhysRevD.85.083002
  [arXiv:1108.5512 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevD.85.083002;%%
  %57 citations counted in INSPIRE as of 10 Feb 2018  
  
%\cite{Springel:2005mi}
\bibitem{c}
  V.~Springel,
  %``The Cosmological simulation code GADGET-2,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 364} (2005) 1105
  doi:10.1111/j.1365-2966.2005.09655.x
  [astro-ph/0505010].
  %%CITATION = doi:10.1111/j.1365-2966.2005.09655.x;%%
  %2681 citations counted in INSPIRE as of 10 Feb 2018


